Operadic approach to wall-crossing

Wall-crossing phenomena are ubiquitous in many problems of algebraic geometry and theoretical physics. Various ways to encode the relevant information and the need to track the changes under the variation of parameters lead to rather complicated transformation rules and non-trivial combinatorial problems. In this paper we propose a framework, reminiscent of collections and plethysms in the theory of operads, that conceptualizes those transformation rules. As an application we obtain new streamlined proofs of some existing wall-crossing formulas as well as some new formulas related to attractor invariants.

==> commands_new.tex <==
\RequirePackage{amsmath,amssymb}%,amsthm}
\RequirePackage{etoolbox,bbm,xspace}
\RequirePackage{version,xparse}
%\RequirePackage[a4paper,margin=1.35in]{geometry}

%%%% Theorem environments
\ifx\notheorems\undefined
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{conjecture}[theorem]{Conjecture}
\theoremstyle{definition}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{exercise}[theorem]{Exercise}
\theoremstyle{remark}
\newtheorem{rmr}[theorem]{Remark}
%\newtheorem{question}[theorem]{Question}
%\AtEndEnvironment{remark}{\hfill$\lozenge$}
%\AtEndEnvironment{example}{\hfill$\lozenge$}
\fi

%%%% Auxiliary commands
\def\mat#1{\ensuremath{#1}\xspace}
\def\dmat#1#2{\gdef#1{\mat{#2}}}
\def\csdmat#1#2{\csdef{#1}{\mat{#2}}}
\def\redef#1{\csletcs{t@#1}{#1}\csdmat{#1}{\csuse{t@#1}}}
\def\opr#1#2{\dmat#1{\operatorname{#2}}}
\def\opra#1#2{\csdmat{#1}{\operatorname{#2}}}
\def\oper#1{\csdmat{#1}{\operatorname{#1}}}
\def\DMO{\opr}
\makeatletter
\def\forlist#1#2{\@xp\forcsvlist\@xp{\@xp#1\@xp}\@xp{#2}}
% usage: \forlist\command\list
\makeatother

%%%% Operators. Usage: \GL
\forcsvlist\oper{
Vect,Mod,Rep,Ab,Grp,Com,Set,Top,Sch,Coh,Qcoh,Ob,Ring,Alg,
Map,Hom,End,Aut,Ext,Cat,Sh,Ind,RHom,Fun,Var,rad,
Ker,Im,deg,Tr,det,rk,diag,im,coker,tr,cone,add,
sk,cosk,colim,Res,Gal,Coker,dlog,
GL,SL,PGL,Gr,Lib,Conv,Sol,Tor,
Max,Spec,Ass,Ann,Quot,Pic,Sym,MHS,MHM,
td,ch,Supp,supp,vol,trdeg,lc,NS,Loc,Iso,per,gr,Der,Lie,
Log,Exp,Pow,ord,lcm,VB,Hilb,cl,SU,SO,Ad,ad,id}
\opr\Id{id}
\opr\lHom{\lb{Hom}}
\opr\lAut{\lb{Aut}}
\opr\lIso{\lb{Isom}}
\opr\hgt{ht}
\opr\chr{char}
\opr\udim{\mathbf{dim}}
\opr\cls{\mathsf{cl}}
\opr\mmod{mod}
\opr\Et{\mathsf{Et}}
\def\gl{\mathfrak{gl}}
\def\sl{\mathfrak{sl}}
\def\su{\mathfrak{su}}
\def\so{\mathfrak{so}}
\oper{sgn}\def\sign{\sgn}


%%%% Symbols
\def\mto{\mapsto}
\def\xto{\xrightarrow}
\def\lto{\leftarrow}
\def\xlto{\xleftarrow}
\def\emb{\hookrightarrow}
\def\lemb{\hookleftarrow}
\def\onto{\twoheadrightarrow}
\def\isoto{\xto{\,\smash{ 
	\raisebox{-3pt}{\ensuremath{\scriptstyle\sim}}
}\,}}
\dmat\es{\varnothing}%{\emptyset}
\def\bs{\backslash}
\def\sbs{\subset}
\def\sps{\supset}
\redef{iff}
\dmat\imp{\implies}
\dmat\xx{\times}
\dmat\dd{\partial}
\def\pd#1{\frac\dd{\dd#1}}
\def\iso{\simeq}
\def\ms{\backslash}
\def\bi{\mathbf i}
\def\bop{\bigoplus}
\def\ilim{\varprojlim} %inverse limit
\def\dlim{\varinjlim} %direct limit
\def\ts{\otimes}
\def\bts{\bigotimes}
\def\lb{\underline}
\def\ub{\overline}
\def\ubar#1{\mkern1.5mu\overline%
	{\mkern-1.5mu#1\mkern-1.5mu}\mkern1.5mu}
\def\oh{{\frac12}}
\dmat\Gm{\mathbb G_{\mathrm m}}
\dmat\one{\mathbbm1}
\def\qt{\delimiter"502F30E\mathopen{}} %/correct spacing
\def\dlim{\varinjlim} %direct limit
\def\ilim{\varprojlim} %inverse limit
\def\partof{\vdash}
\def\what{\widehat}
\def\tl{\tilde}
\def\wtl{\widetilde}
\def\inv{^{-1}}
\def\dual{^{\vee}}
\def\trp{^{\mathsf T}} %transpose
\dmat\pt{\mathbf{pt}}
\def\op{\mathrm{op}}
\def\st{\mathrm{s}}
\def\sst{\mathrm{ss}}
\def\nil{\mathsf {nil}}
\def\et{\mathrm{et}}
\def\ri{\mathrm i}
\def\sep{\mathrm{sep}}
\def\ab{\mathrm{ab}}
\def\top{\mathrm{top}}
\def\Ta{T^{\mathrm a}} %tensor algebra
\def\Tc{T^{\mathrm c}} %tensor coalgebra
\dmat\bul{\bullet}
\newdimen\bulh\settoheight\bulh{\bul}
\def\sbul{{\hspace{.5pt}\raisebox{.5\bulh}{%
	\scalebox{.5}{\raisebox{-.5\bulh}{\bul}}%
}}}%small bullet
\def\GIT{/\!\!/}
\def\qbinom{\genfrac{[}{]}{0pt}{}}
\def\ac{{\tiny\raisebox{2pt}{\textup{!`}}}}%anti-shriek
\newlength{\mylength}

\def\xmto#1{\,\tikz{
	\settowidth{\mylength}{\mat{#1}}
	\draw(0,1mm)--(0,-1mm);
	\draw[->](0,0)--(2\mylength,0)
	node[above,midway]{\mat{#1}};
	}\,}
\def\upc{\tikz{\draw[->,>=latex'](0,0)--(0,.3)}}
%requires \usetikzlibrary{arrows}
\def\upc#1{\left\uparrow#1\right.}%upper closure
\def\loc#1{\left\downarrow#1\right.}%lower closure


%%%% Aphabets: \bA,\cA,\fA,\bfA,\sA
\def\defbb#1{\csdmat{b#1}{\mathbb{#1}}}
\def\defcal#1{\csdmat{c#1}{\mathcal{#1}}}
\def\deffrak#1{\csdmat{f#1}{\mathfrak{#1}}}
\def\defbf#1{\csdmat{bf#1}{\mathbf{#1}}}
\def\defsf#1{\csdmat{s#1}{\mathsf{#1}}}
\def\defall#1{\defbb{#1}\defcal{#1}\deffrak{#1}\defbf{#1}\defsf{#1}}
\forcsvlist\defall{A,B,C,D,E,F,G,H,I,J,K,L,M,N,O,P,Q,R,S,T,U,V,W,X,Y,Z}
\forcsvlist\deffrak{a,b,c,d,e,f,g,h,j,k,l,m,n,o,p,q,r,s,t,u,v,w,x,y,z}
\def\defbl#1{\csdmat{b#1}{\mathbf{#1}}} %lower case
\forcsvlist\defbl{a,b,c,d,e,g,h,i,j,k,l,n,o,p,q,r,s,t,u,v,w,x,y,z}
%\dmat\bk{\mathbbm k}
\dmat\bk{\Bbbk}

%%%% Greek letters
\dmat\al\alpha
\dmat\be\beta
\dmat\ga\gamma
\dmat\de\delta
\dmat\la\lambda
\dmat\ta\tau
\dmat\hi\chi
\dmat\eps\varepsilon
\dmat\vi\phi
\dmat\te\theta
\dmat\ksi\xi
\dmat\si\sigma
\dmat\om\omega
\dmat\Ga\Gamma
\dmat\La\Lambda
\dmat\De\Delta
\dmat\Om\Omega
\dmat\Si{\Sigma}
\dmat\ze\zeta
\dmat\Te{\Theta}
\dmat\Na{\nabla}
\dmat\kp{\kappa}
\forcsvlist\redef{Phi,Psi,pi,mu,nu}

%%%% Structures
\def\set#1{\mat{\left\{#1\right\}}}
\def\sets#1#2{\left\{\left.#1\ \right\vert#2\right\}}
\def\ang#1{\mat{\left\langle#1\right\rangle}}
\def\angs#1#2{\ang{#1\rcol#2}}
\def\rbr#1{\left(#1\right)}
\def\sbr#1{\left[#1\right]}
\def\bra#1{\langle#1|}
\def\ket#1{|#1\rangle}
\def\n#1{\left\lvert#1\right\rvert}
\def\nn#1{\left\lVert#1\right\rVert}
\def\eq#1{\begin{equation}#1\end{equation}}
\def\ov#1#2{{\substack{#1\\#2}}} % #1 over #2
\def\pser#1{[\![#1]\!]} %formal power series [[#1]]
\def\lser#1{(\;\!\!\!(#1)\!\!\!\;)} %formal Laurent series ((#1))
\def\pmat#1{\begin{pmatrix}#1\end{pmatrix}}
\def\vmat#1{\begin{vmatrix}#1\end{vmatrix}}
\def\smat#1{\left(\begin{smallmatrix}#1\end{smallmatrix}\right)}
\def\matr#1{\begin{matrix}#1\end{matrix}}
\def\pmatv#1#2{\left(\matr{#1}
	\hspace{.5ex}\middle|\hspace{.3ex}
	\matr{#2}\right)}
%\def\matr{\pmat}
\def\nop#1{\left.\col#1\col\right.}%normal oper product

%%%% Diff
\def\br{\ \vspace{-.5ex}} %break after itemize
\def\dir#1#2{\noindent\textbf{(#1)$\implies$(#2).}}
\def\clm#1{\noindent\textbf{(#1)}\xspace} %claim, \cl should be used for classes
\def\lqq{\lq\lq}
\def\rqq{\rq\rq\xspace}
\def\qq#1{\lqq#1\rqq}
\def\tpdf{\texorpdfstring} %hyperref
\def\hl{\noindent\rule{\textwidth}{1pt}}

%%%% Words and phrases
\def\ie{i.e.\@\xspace} %id est
\def\cf{cf.\@\xspace} %confer
\def\eg{e.g.\@\xspace} %exempli gratia
%\def\fd{f.d.\@\xspace} % used for \mathfrak{d}
\def\etale{\'etale\xspace}
\def\qis{quism\xspace} %quasi-isomorphism
\def\wrt{with respect to\xspace}
\def\hint{\noindent\textbf{Hint:}\xspace}
\def\Wlog{Without loss of generality\xspace}
\def\tfae{the following are equivalent\xspace}
\def\nbd{neighborhood\xspace}

%%%% Citations
\def\defcite#1#2{%\defcite\moz{mozgovoy_DT}
	\DeclareDocumentCommand{#1}{o}
		{\IfValueTF{##1}{\cite[##1]{#2}}{\cite{#2}}\xspace}
}

%%%% Colons
%\usepackage{mathtools}
%\mathtoolsset{centercolon}
% : is math active with mathtools "centercolon"
\edef\col{\mathchar\the\mathcode`:} %ordinary :
\patchcmd\colon{:}{\col}{}{} %avoid the mention of :
\makeatletter
\begingroup
\catcode`:=\active 
\gdef:{\@ifnextchar={\col}\colon}
\endgroup
\def\rcol{\col}
\AtBeginDocument{\mathcode`:="8000}

%%% Redefine = so that =: works
\edef\latexequal{\mathchar\the\mathcode`=}
\begingroup
\catcode`==\active
\gdef={\latexequal\@ifnextchar:{\afterassignment\col\let\next}{}}
\endgroup
\AtBeginDocument{\mathcode`=="8000}

%%%% Indexed definition \idef{name}{optional name}
\DeclareDocumentCommand{\idef}{mo}{%
	\ifmmode#1\else\textit{#1}\fi%
	\IfValueTF{#2}{\index{#2}}{\index{#1}}%
}

%%%%% Tikz commands
\newenvironment{ctikzcd}
	{\center\tikzcd}{\endtikzcd\endcenter}
\newenvironment{ctikz}
	{\center\tikzpicture}{\endtikzpicture\endcenter}

%custom theorem, can be used to list axioms (with labels)
\theoremstyle{plain}
\newtheorem{innercustomthm}{}
\newenvironment{customthm}[1]
  {\def\theinnercustomthm{#1}\innercustomthm}
  {\endinnercustomthm}

\DeclareDocumentCommand\sec{o}{
	\IfValueTF{#1}{\subsection{#1}}
			{\subsection{}\hspace{-1ex}}}

